WATCHDOG: an ontology-aWare risk AssessmenT approaCH via object-oriented DisruptiOn Graphs

When considering risky events or actions, we must not downplay the role of involved objects: a charged battery in our phone averts the risk of being stranded in the desert after a flat tyre, and a functional firewall mitigates the risk of a hacker intruding the network. The Common Ontology of Value and Risk (COVER) highlights how the role of objects and their relationships remains pivotal to performing transparent, complete and accountable risk assessment. In this paper, we operationalize some of the notions proposed by COVER -- such as parthood between objects and participation of objects in events/actions -- by presenting a new framework for risk assessment: WATCHDOG. WATCHDOG enriches the expressivity of vetted formal models for risk -- i.e., fault trees and attack trees -- by bridging the disciplines of ontology and formal methods into an ontology-aware formal framework composed by a more expressive modelling formalism, Object-Oriented Disruption Graphs (DOGs), logic (DOGLog) and an intermediate query language (DOGLang). With these, WATCHDOG allows risk assessors to pose questions about disruption propagation, disruption likelihood and risk levels, keeping the fundamental role of objects at risk always in sight.

==> algorithms/BDDs_from_ODG_lOne.tex <==
% !TEX root =  main.tex
\begin{breakablealgorithm}
\small
        \caption{Compute $\BDDlOne$ from \ODG $G$ and $\lOne$}
    \begin{algorithmic}[1]
        \State \textbf{Input}: \ODG $\odg$, formula $\lOne$, \textbf{Output:} \BDD $\BDDlOne$, \textbf{Method:}
        \If{$\lOne$ = $a$}
            \If{$a \in N_A$}   \textbf{return} $\Trans_{A}(a)$
            \ElsIf{$a \in N_F$} \textbf{return} $\Trans_{F}(a)$
            \ElsIf{$a \in OP$} \textbf{return} $\bddOp(a)$
            \EndIf
        \ElsIf{$\lOne$ = $\lnot\lOne'$} \textbf{return} $\contour{black}{\BDDnot}\left(\Cref{alg:BDDs_from_ODG_lOne}(\odg, \lOne') \right)$
        \ElsIf{$\lOne$ {=} $\lOne'\land\lOne''$} \textbf{return} $\Cref{alg:BDDs_from_ODG_lOne}(\odg, \lOne') \contour{black}{\BDDand} \Cref{alg:BDDs_from_ODG_lOne}(\odg, \lOne'')$
        \ElsIf{$\lOne$ = $\lOne'[a_i\mapsto bool]$}  \textbf{return} $\textsc{Restrict}(\Cref{alg:BDDs_from_ODG_lOne}(\odg, \lOne'), x_i, bool \in \BB)$
        \Else{ \textcolor{gray}{\,\,\,\,\,\,$//  \text{ }\lOne$ = $\opMRS(\lOne')$}} \State \textbf{return} $\Cref{alg:BDDs_from_ODG_lOne}(\odg, \lOne') \contour{black}{\BDDand} (\contour{black}{\BDDNExists} \tVprime . (\tVprime $ \contour{black}{$\subset$} $ \tV) \contour{black}\BDDand\Cref{alg:BDDs_from_ODG_lOne}(\odg, \lOne')[\tV$ \contour{black}{$\curvearrowright$} $ \tVprime])$
        \EndIf
    \end{algorithmic}
	\label{alg:BDDs_from_ODG_lOne}
\end{breakablealgorithm}

